A Simple Single Slot Finality Protocol For Ethereum

Currently, Gasper, the implemented consensus protocol of Ethereum, takes between 64 and 95 slots to finalize blocks. Because of that, a significant portion of the chain is susceptible to reorgs. The possibility to capture MEV (Maximum Extractable Value) through such reorgs can then disincentivize honestly following the protocol, breaking the desired correspondence of honest and rational behavior. Moreover, the relatively long time to finality forces users to choose between economic security and faster transaction confirmation. This motivates the study of the so-called single slot finality protocols: consensus protocols that finalize a block in each slot and, more importantly, that finalize the block proposed at a given slot within such slot. In this work we propose a simple, non-blackbox protocol that combines a synchronous dynamically available protocol with a partially synchronous finality gadget, resulting in a consensus protocol that can finalize one block per slot, paving the way to single slot finality within Ethereum. Importantly, the protocol we present can finalize the block proposed in a slot, within such slot.

==> algorithms/protocol.tex <==
\begin{algo}[htb!]
\small
\begin{numbertabbing}\reset

xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=xxxx\=MMMMMMMMMMMMMMMMMMM\=\kill
  \textbf{State} \label{}\\
  \> \(\V_i \gets \{\B_{\text{genesis}}\} \): view of validator $v_i$ \label{}\\
  \> \(\B_i \gets \emptyset \): buffer of validator $v_i$  \label{}\\
  \> \(\chain_i \gets B_{\text{genesis}}\): canonical chain of validator $v_i$ \label{}\\  
  \> \(t \gets 0\): the current slot \label{}\\
  \> \(r \gets 0\): the current round \label{}\\
  \textsc{propose}\\
  \textbf{at} $r=4\Delta t$ \textbf{do} \label{} \\
  \> \textbf{if} $v_i = v_p^t$ \textbf{then} \label{}\\
  \>\>$\V_i \gets \V_i \cup \B_i$, $\B_i \gets \emptyset$ , $B' \gets \hfc(\V_i, t)$ \label{line:alg2-fc1}\\
  \>\> $B \gets \mathsf{NewBlock}(B')$, $\chain_i \gets B$ \label{}\\
  \>\> send message [\textsc{propose}, $B$, $\V_i\,\cup \{B\}$, $t$, $v_i$] through gossip \label{}\\
     \textsc{Head-vote}\\
     \textbf{at} $r=4\Delta t + \Delta$ \textbf{do} \label{}\\
     \> $\chain_i \gets \hfc(\V_i, t)$ \label{line:alg2-fc2}\\
     \> send message [\textsc{head-vote}, $\hfc(\V_i, t)$, $t$, $v_i$] through gossip \label{line:alg2-fc3}\\
    \textsc{Confirm and ffg-vote}\\
     \textbf{at} $r=4\Delta t + 2\Delta$ \textbf{do} \label{}\\
     \> $B_{\text{fast}} \gets \genesis$ \label{} \\
     \> $S_{\text{fast}} \gets \{B \prec \chain_i\colon |\{v_i\colon \exists B' \succ B  \ [\textsc{head-vote}, B', t, v_i] \in \B_i \}| \geq \frac{2}{3}n\}$ \label{} \\
     \> \textbf{if} $S_{\text{fast}} \neq \emptyset$ \textbf{then}: \label{}\\
    \>\> $B_{\text{fast}} \gets \underset{S_{\text{fast}}}{\text{arg max}} |B|$ \label{}\\
    \> \textbf{if} $\neg (B_{\text{fast}} \prec  \chainava_i \land \chain_i^{\lceil \kappa} \prec \chainava_i) $ \textbf{then}: \label{}\\
     \>\> $\chainava_i \gets \underset{\chain \in \{\chain_i^{\lceil \kappa}, B_{\text{fast}}\}}{\text{arg max}} |\chain|$ \label{}\\
    \>  $\C_{\text{target}} \gets (\underset{B \in \{LJ_i, \chainava_i\}}{\text{arg max}}|B|,t)$\label{line:set-target-checkpoint}\\
     \> send message [\textsc{ffg-vote}, $\LJ_i$, $\C_{\text{target}}$, $v_i$] through gossip  \label{line:cast-ffg-vote}\\
    \textsc{merge}\\
     \textbf{at} $r=4\Delta t + 3\Delta$ \textbf{do} \label{}\\
     \> $\V_i \gets \V_i \cup \B_i$ \label{}\\
       \> $\B_i \gets \emptyset$ \label{}\\
    \textbf{upon} receiving a gossiped message
    [\textsc{propose}, $B$, $\V$, $t$, $v_p^t$] \textbf{do} \label{}\\
    \> $\B_i \gets \B_i \cup \{B\}$ \label{}\\  
    \> \textbf{if} $r \in [4\Delta t, 4\Delta t + \Delta]$ \textbf{then} \label{}\\
    \>\> $\V_i \gets \V_i \cup \V$ \label{}\\
    \textbf{upon} receiving a gossiped message $V = $ [\textsc{head-vote}, $B$, $t'$, $v_i$] from \(v_i\) \textbf{do} \label{}\\
    \> $\B_i \gets \B_i \cup \{V\}$ \label{}\\  
    \textbf{upon} receiving a gossiped block $B = $ (\textsc{block}, $b$, $t'$, $v_i$) from \(v_i\) \textbf{do} \label{}\\
    \> $\B_i \gets \B_i \cup \{B\}$ \label{}\\
    [-5ex]
\end{numbertabbing}
\caption{Single slot finality protocol for validator $v_i$}
\label{alg:pvm-generic}
\end{algo}



==> figures/black-box-slot-structure.tex <==

\begin{tikzpicture}[x=2cm]
    % \small
    % \footnotesize

    \draw [dashed] (-0.4,0) -- (0,0);
    \draw [-Latex] (0,0) -- (5.5,0) node [right] {Time};

    % \draw [] (-1,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $3\Delta(t-1)+2\Delta$};
    \draw [] (0,0) -- ++(0,0.2) -- ++(0,-0.4) node [below left] {Slot $(t-1)$};
    \draw [] (2,0) -- ++(0,0.1) -- ++(0,-0.2);
    \draw [] (3,0) -- ++(0,0.1) -- ++(0,-0.2);
    \draw [] (4,0) -- ++(0,0.1) -- ++(0,-0.2);
    \draw [] (5,0) -- ++(0,0.2) -- ++(0,-0.4) node [below right] {Slot $t+1$};
    % \draw [] (5,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta (t+1) + 1\Delta$};
    % \draw [] (4,0) -- ++(0,0.2) -- ++(0,-0.4);
    
    \draw [densely dotted] (0,0) -- ++(0,-1.6);
    \draw [densely dotted] (5,0) -- ++(0,-1.6);
    \draw [densely dotted] (2,0) -- ++(0,-0.8);
    \draw [densely dotted] (4,0) -- ++(0,-0.8);

    % \node at (-0.5,-0.6) {...};
    % \node at (4.5,-0.6) {...};
    \begin{scope}[yshift=-2cm]
        \draw [Latex-Latex] (0,0) -- ++(5,0) node [midway,below] {slot $t$};
    \end{scope}

    \begin{scope}[yshift=-1cm]
        \draw [Latex-Latex] (0,0) -- ++(2,0) node [midway,below] {DA protocol slot} node [midway, above] {$k \Delta$};
        \draw [Latex-Latex] (2,0) -- ++(2,0) node [midway,below] {Casper-FFG} node [midway, above] {$2 \Delta$};
        \draw [Latex-Latex] (4,0) -- ++(1,0) node [midway,below] {View-merge} node [midway, above] {$\Delta$};
    \end{scope}


    \draw [Latex-,densely dotted] (0,0) ++(0,0.8) -- ++(0,3) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {\textbf{Slot $t$ proposer:} merge FFG buffer into local view, propose FFG view; \\ Throughout the DA protocol slot, perform proposer duties in the DA protocol};
    
    \draw [Latex-,densely dotted] (2,0) ++(0,0.8) -- ++(0,2) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {cast first FFG votes};

    \draw [Latex-,densely dotted] (3,0) ++(0,0.8) -- ++(0,1.5) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge first FFG votes into local view; cast second FFG votes};

    \draw [Latex-,densely dotted] (4,0) ++(0,0.8) -- ++(0,1) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge FFG buffer into local view};


\end{tikzpicture}



==> figures/slot-structure-chained.tex <==

\begin{tikzpicture}[x=2cm]
    % \small
    % \footnotesize

    \draw [dashed] (-0.4,0) -- (0,0);
    \draw [-Latex] (0,0) -- (4.5,0) node [right] {Rounds};

    % \draw [] (-1,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $3\Delta(t-1)+2\Delta$};
    \draw [] (0,0) -- ++(0,0.2) -- ++(0,-0.4) node [pos=0,above] {\footnotesize $4\Delta t$} node [below left] {Slot $(t-1)$};
    \draw [] (1,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 1\Delta$};
    \draw [] (2,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 2\Delta$};
    \draw [] (3,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 3\Delta$};
    \draw [] (4,0) -- ++(0,0.2) -- ++(0,-0.4) node [pos=0,above] {\footnotesize $4\Delta (t+1)$} node [below right] {Slot $t+1$};
    
    \draw [densely dotted] (0,0) -- ++(0,-1);
    \draw [densely dotted] (4,0) -- ++(0,-1);

    % \node at (-0.5,-0.6) {...};
    % \node at (4.5,-0.6) {...};
    \begin{scope}[yshift=-1cm]
        \draw [Latex-Latex] (0,0) -- ++(4,0) node [midway,below] {slot $t$};
    \end{scope}

    \draw [Latex-,densely dotted] (0,0) ++(0,0.8) -- ++(0,2.5) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {\textbf{Slot $t$ proposer:} merge buffer into local view; propose block and view};
    
    \draw [Latex-,densely dotted] (1,0) ++(0,0.8) -- ++(0,2) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge proposed view into local view; cast head vote and FFG vote together};
    
    \draw [Latex-,densely dotted] (2,0) ++(0,0.8) -- ++(0,1.5) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {run optimistic fast confirmation rule};

    \draw [Latex-,densely dotted] (3,0) ++(0,0.8) -- ++(0,1) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge buffer into local view; cast finality vote};


\end{tikzpicture}



==> figures/slot-structure.tex <==

\begin{tikzpicture}[x=2cm]
    % \small
    % \footnotesize

    \draw [dashed] (-0.4,0) -- (0,0);
    \draw [-Latex] (0,0) -- (4.5,0) node [right] {Rounds};

    % \draw [] (-1,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $3\Delta(t-1)+2\Delta$};
    \draw [] (0,0) -- ++(0,0.2) -- ++(0,-0.4) node [pos=0,above] {\footnotesize $4\Delta t$} node [below left] {Slot $(t-1)$};
    \draw [] (1,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 1\Delta$};
    \draw [] (2,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 2\Delta$};
    \draw [] (3,0) -- ++(0,0.1) -- ++(0,-0.2) node [pos=0,above] {\footnotesize $4\Delta t + 3\Delta$};
    \draw [] (4,0) -- ++(0,0.2) -- ++(0,-0.4) node [pos=0,above] {\footnotesize $4\Delta (t+1)$} node [below right] {Slot $t+1$};
    
    \draw [densely dotted] (0,0) -- ++(0,-1);
    \draw [densely dotted] (4,0) -- ++(0,-1);

    % \node at (-0.5,-0.6) {...};
    % \node at (4.5,-0.6) {...};
    \begin{scope}[yshift=-1cm]
        \draw [Latex-Latex] (0,0) -- ++(4,0) node [midway,below] {slot $t$};
    \end{scope}

    \draw [Latex-,densely dotted] (0,0) ++(0,0.8) -- ++(0,2.5) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {\textbf{Slot $t$ proposer:} merge buffer into local view; propose block and view};
    
    \draw [Latex-,densely dotted] (1,0) ++(0,0.8) -- ++(0,2) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge proposed view into local view; cast head vote};
    
    \draw [Latex-,densely dotted] (2,0) ++(0,0.8) -- ++(0,1.5) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {run optimistic fast confirmation rule; cast FFG vote};

    \draw [Latex-,densely dotted] (3,0) ++(0,0.8) -- ++(0,1) -- ++(0.1,0) node [align=left,right,font=\scriptsize] {merge buffer into local view; cast finality vote};


\end{tikzpicture}



==> missing-proofs.tex <==
\section{Missing proofs}
\label{appendix:missing-proofs}

\begin{proof}[Proof of Theorem~\ref{thm:equivalence}]
Since the only difference between the two protocols is the fork-choice function $\FC$, the sequences of outputs correspond as long as the outputs of $\hfc$ and $\rlmdghost$ obtained by active validators are always the same in the two executions. $\FC$ is used only twice in Algorithm~\ref{alg:pvm-generic}, in Line~\ref{line:alg2-fc1} for proposing, and in Lines~\ref{line:alg2-fc2}-\ref{line:alg2-fc3}, with the same input, for broadcasting a \textsc{head-vote}. We are going to prove by induction that the canonical chain of an active validator \emph{at any voting round} is the same in both executions. Since Line~\ref{line:alg2-fc2} sets $\chain_i \gets \FC(V_i, t)$, and this value is the same as in Line~\ref{line:alg2-fc3}, we only need to show that the fork-choice output in Line~\ref{line:alg2-fc1} coincides in the two executions as well. In Line~\ref{line:alg2-fc3}, an honest validator uses the fork-choice output to construct their \textsc{head-vote}s, so \textsc{head-vote}s correspond in both executions. Moreover, the view-merge property applies in both executions, so honestly proposed blocks correspond to the honest \textsc{head-vote}s from their slot. Therefore, \textsc{head-vote}s coinciding in the two executions implies that honestly proposed blocks coincide as well. Since honestly proposed blocks extend the output of the fork-choice at Line~\ref{line:alg2-fc1}, this output is then also the same in both executions, completing the proof. We now carry out the induction.

\textbf{Induction hypothesis:} At any slot $t' \leq t$ and for $r = 4\Delta t' + \Delta$, $\chain_i^r$ coincides in both executions, for any active validator $i$.

\textbf{Base case:} In rounds $[0, \Delta]$, the two executions are exactly the same, because the only justified checkpoint is \genesis, so $\hfc = \rlmdghost$. Therefore, the statement holds for $t = 0$.

\textbf{Inductive step:} Suppose now that the statement holds for~$t$, and consider round $r = 4\Delta (t+1) + \Delta$. Consider an active validator~$v_i$ with view $\V_i$ at round $r$, and latest justified block $B = LJ(\V_i)$. Let~$t'$ be minimal such that there exists a justified checkpoint~$\C = (B, t')$, \ie, slot~$t'$ is the first slot in which block~$B$ was justified. The supermajority link with target~$\C$ contains at least one FFG vote from an honest validator~$v_k$. By minimality of~$t'$, $B$ could not have been already justified in the view of~$v_k$ when broadcasting an FFG vote at slot~$t'$. Therefore, by Lines~\ref{line:set-target-checkpoint}-\ref{line:cast-ffg-vote} of Algorithm~\ref{alg:pvm-generic}, it must be the case that $B \prec \chainava_k$ at round $4\Delta t' + 2\Delta$, \ie, that it had been confirmed by~$v_k$. If it was fast confirmed at a slot $\leq t'$, then, in the execution with $\FC = \rlmdghost$, Theorem~\ref{thm:fast-reorg-resilience} implies that $B \prec \chain_j^{r'}$ for all active validators $v_j$ at any round $r' \geq 4\Delta (t'+1) + \Delta$, and so in particular that $B \prec \chain_i^r$, since $t > t'$. If instead $B \prec \chain_k^{\lceil \kappa}$ at round $4\Delta t' + 2\Delta$, \ie, $B$ is confirmed by $v_k$ due to being $\kappa$-deep in its canonical chain, then with overwhelming probability there exists a pivot slot $t'' \in [t'-\kappa, t')$ (Lemma 3~\cite{rlmd}), with proposed block~$B'$. In the execution with $\FC = \rlmdghost$, $\eta$-reorg-resilience then implies that $B' \prec \chain_j^{r'}$ for all active validators $v_j$ at any round $r' \geq 4\Delta t'' + \Delta$. In particular, $B' \prec \chain_k^{r'}$ at round $r' = 4\Delta t' + 2\Delta$, and $B' \prec \chain_i^r$. The former implies $B \prec B'$, since $B.t \leq t'-\kappa \leq B'.t$, and we then have $B \prec B' \prec \chain_i^{r}$. 

Anyway, regardless of how~$B$ has been confirmed by $v_k$, we have $B \prec \chain_i^r$. Therefore, $LJ(\V_i) = B \prec \rlmdghost(\V_i, t+1)$, which in turn implies $\rlmdghost(\V_i, t+1) = \rlmdghost \circ\,\FIL_{\text{FFG}}(\V_i, t+1) = \hfc(\V_i, t+1)$. Therefore, after~$v_i$ updates its canonical chain $\chain_i$ at round $r$ by setting $\chain_i \gets \FC(\V, t+1)$, with~$\FC$ dependent on the execution,~$\chain_i$ is the same in both executions.
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:accountable-safety}]
We assume throughout that there are no double justifications, \ie, there are no checkpoints $\C \neq \C'$ with $\C.t = \C'.t$, and we refer to this as the non-equivocation assumption. If that's not the case, clearly $\geq \frac{n}{3}$ validators are slashable for violating $\mathbf{E_1}$. Consider two conflicting finalized blocks $B$ and $B'$. By definition, there are also finalized checkpoints $\C$ and $\C'$ with $B = \C.B$, $B' = \C'.B$. Say $\C$ is finalized by the chain of supermajority links (\genesis, $0) \to \C_1 \dots \to \C_k = \C \to \C_{k+1}$, with $\C_{k+1}.t = \C.t + 1$, and $\C'$ by the chain (\genesis, $0) \to \C'_1 \dots \to \C'_{k'} = \C' \to \C'_{k'+1}$, with $\C'_{k'+1}.t = \C'.t + 1$.  Let $t_i = \C_i.t$, and $t'_i = \C'_i.t$. By the non-equivocation assumption, $t_k \neq t'_k$, and without loss of generality we take $t_k < t'_k$. Let $j = \min\{i\leq k'\colon t_k < t'_i\}$, so $t_k < t'_j \leq t'_{k'}$, and $t'_{j-1} \leq t_k$ by minimality of $t'_j$. By the non-equivocation assumption, $t'_j = t_{k+1}$ implies that $\C_{k+1} = \C'_j$. We then have $B = \C.B \prec \C_{k+1}.B = \C'_{j}.B \prec \C'.B = B'$, contradicting that $B$ and $B'$ are conflicting. Therefore, $t'_j > t_k + 1 = t_{k+1}$ as well. Similarly, $t'_{j-1} < t_k$. Therefore, we have $t'_{j-1} < t_k < t_{k+1} < t'_{k}$, \ie, $\C'_{j-1}.t < \C_k.t < \C_{k+1}.t < \C'_j.t$. The intersection of the two sets of voters of the supermajority links $\C_{k} \to \C_{k+1}$ and $\C'_{j-1} \to \C'_j$ contains at least $\frac{n}{3}$ validators, which are then slashable for violating $\mathbf{E_2}$. 
\end{proof}


\begin{proof}[Proof of Theorem~\ref{thm:acc-saf-ack}]
The proof largely follows that of Theorem~\ref{thm:accountable-safety}. We again consider two conflicting finalized blocks $B$ and $B'$, and corresponding finalized checkpoints $\C$ and $\C'$. Regardless of whether finalization is through a supermajority link or a supermajority acknowledgment, $\C$ and $\C'$ have to be justified, by chains of supermajority links (\genesis, $0) \to \C_1 \dots \to \C_k = \C$ and (\genesis, $0) \to \C'_1 \dots \to \C'_{k'} = \C'$. Let $t_i = \C_i.t$, and $t'_i = \C'_i.t$. By the non-equivocation assumption considered in Theorem~\ref{thm:accountable-safety}, we again have $t_k \neq t'_k$, and without loss of generality we take $t_k < t'_k$. As before, we let $j = \min\{i\leq k'\colon t_k < t'_i\}$, so $t_k < t'_j \leq t'_{k'}$, and $t'_{j-1} \leq t_k$ by minimality of $t'_j$. Moreover, also by the non-equivocation assumption, $t'_{j-1} < t_k$. If $\C$ is finalized through a supermajority link, the proof of Theorem~\ref{thm:accountable-safety} already shows that at least $\frac{n}{3}$ validators must have violated $\mathbf{E_2}$, and it is still applicable here because it does not use the last supermajority link in the chain finalizing $\C'$ (which may or may not exist here). If instead $\C$ is finalized through a supermajority acknowledgment, \ie, there are $\frac{2}{3}n$ acknowledgments of $\C$, then at least $\frac{n}{3}$ validators have violated $\mathbf{E_3}$, because $\C'_{j-1}.t < \C.t < \C'_j.t$.
\end{proof}
